Digital Twins and Testbeds for Supporting AI Research with Autonomous Vehicle Networks

Digital twins (DTs), which are virtual environments that simulate, predict, and optimize the performance of their physical counterparts, hold great promise in revolutionizing next-generation wireless networks. While DTs have been extensively studied for wireless networks, their use in conjunction with autonomous vehicles featuring programmable mobility remains relatively under-explored. In this paper, we study DTs used as a development environment to design, deploy, and test artificial intelligence (AI) techniques that utilize real-world (RW) observations, e.g. radio key performance indicators, for vehicle trajectory and network optimization decisions in autonomous vehicle networks (AVN). We first compare and contrast the use of simulation, digital twin (software in the loop (SITL)), sandbox (hardware-in-the-loop (HITL)), and physical testbed (PT) environments for their suitability in developing and testing AI algorithms for AVNs. We then review various representative use cases of DTs for AVN scenarios. Finally, we provide an example from the NSF AERPAW platform where a DT is used to develop and test AI-aided solutions for autonomous unmanned aerial vehicles for localizing a signal source based solely on link quality measurements. Our results in the physical testbed show that SITL DTs, when supplemented with data from RW measurements and simulations, can serve as an ideal environment for developing and testing innovative AI solutions for AVNs.

==> acronyms.tex <==
\newacronym{3gpp}{3GPP}{3rd Generation Partnership Project}
\newacronym{5g}{5G NR}{fifth generation new radio}
\newacronym{6g}{6G}{sixth generation}
\newacronym{5gc}{5GC}{5G core}
\newacronym{ai}{AI}{artificial intelligence}
\newacronym{ar}{AR}{augmented reality}
\newacronym{api}{API}{application programming interface}
\newacronym{achem}{ACHEM}{AERPAW Channel Emulator}
\newacronym{aerpaw}{AERPAW}{Aerial Experimentation and Research Platform for Advanced Wireless}
\newacronym{av}{AV}{autonomous vehicle}
\newacronym{avn}{AVN}{autonomous vehicle network}
\newacronym{bs}{BS}{base station}
\newacronym{chem}{CHEM}{channel emulator}
\newacronym{dac}{DAC}{digital-to-analog converter}
\newacronym{darpa}{DARPA}{Defense Advanced Research Projects Agency}
\newacronym{dl}{DL}{downlink}
\newacronym{dt}{DT}{digital twin}
\newacronym{dtn}{DTN}{digital twin network}
\newacronym{enb}{eNB}{E-UTRAN NodeB}
\newacronym{epc}{EPC}{Evolved Packet Core}
\newacronym{fifo}{FIFO}{first-in-first-out}
\newacronym{fpga}{FPGA}{field programmable gate array}
\newacronym{gnb}{gNB}{Next-Generation Node B}
\newacronym{hitl}{HITL}{hardware-in-the-loop}
\newacronym{iot}{IoT}{Internet-of-Things}
\newacronym{ioe}{IoE}{Internet-of-Everything}
\newacronym{itu-t}{ITU-T}{ITU Telecommunication Standardization Sector}
\newacronym{lte}{LTE}{Long-Term Evolution}
\newacronym{ng}{NextG}{next-generation}
\newacronym{ntn}{NTN}{non-terrestrial network}
\newacronym{mmtc}{mMTC}{massive machine-type communications}
\newacronym{otw}{OTW}{over-the-wire}
\newacronym{oran}{O-RAN}{open radio access network}
\newacronym{pci}{PCI}{physical cell identity}
\newacronym{prb}{PRB}{physical resource block}
\newacronym{pt}{PT}{physical twin}
\newacronym{ptv}{PtV}{Physical-to-Virtual}
\newacronym{rf}{RF}{Radio Frequency}
\newacronym{rw}{RW}{real-world}
\newacronym{rsrp}{RSRP}{reference signal received power}
\newacronym{rssi}{RSSI}{received signal strength index}
\newacronym{sdr}{SDR}{software-defined radio}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{sitl}{SITL}{software-in-the-loop}
\newacronym{vr}{VR}{virtual reality}
\newacronym{uav}{UAV}{unmanned aerial vehicle}
\newacronym{ue}{UE}{user equipment}
\newacronym{ul}{UL}{Uplink}
\newacronym{ugv}{UGV}{unmanned ground vehicle}
\newacronym{usrp}{USRP}{universal software radio peripheral}
\newacronym{vtp}{VtP}{Virtual-to-Physical}
\newacronym{xr}{XR}{extended reality} 
\newacronym{qos}{QoS}{quality-of-service}
\newacronym{oac}{OAC}{over-the-air computation}
\newacronym{fl}{FL}{federated learning}

